Human adaptation to adaptive machines converges to game-theoretic equilibria

Adaptive machines have the potential to assist or interfere with human behavior in a range of contexts, from cognitive decision-making to physical device assistance. Therefore it is critical to understand how machine learning algorithms can influence human actions, particularly in situations where machine goals are misaligned with those of people. Since humans continually adapt to their environment using a combination of explicit and implicit strategies, when the environment contains an adaptive machine, the human and machine play a game. Game theory is an established framework for modeling interactions between two or more decision-makers that has been applied extensively in economic markets and machine algorithms. However, existing approaches make assumptions about, rather than empirically test, how adaptation by individual humans is affected by interaction with an adaptive machine. Here we tested learning algorithms for machines playing general-sum games with human subjects. Our algorithms enable the machine to select the outcome of the co-adaptive interaction from a constellation of game-theoretic equilibria in action and policy spaces. Importantly, the machine learning algorithms work directly from observations of human actions without solving an inverse problem to estimate the human's utility function as in prior work. Surprisingly, one algorithm can steer the human-machine interaction to the machine's optimum, effectively controlling the human's actions even while the human responds optimally to their perceived cost landscape. Our results show that game theory can be used to predict and design outcomes of co-adaptive interactions between intelligent humans and machines.

==> fig/tex_cobb.tex <==
\centering
\includegraphics[width=\textwidth]{fig/fig_cobb.pdf}
\caption[Modified Experiments 1, 2 and 3 with non-quadratic costs]{\label{fig:exp-cobb}
\footnotesize
\textbf{Modified Experiments 1, 2 and 3 with non-quadratic costs} ($n=20\times 3$): Non-quadratic costs.
    (\textbf{A}) Gradient descent in action space; decision vector distributions.
(\textbf{B}) Conjectural variation in policy space; decision vector distributions, game theoretic equilibria and best-response functions.
(\textbf{C}) Gradient descent in policy space; decision vector distributions and policy gradient iterations.   
}


==> fig/tex_exp1v5.tex <==
\centering
\includegraphics[width=\textwidth]{fig/fig_exp1v5.pdf}
  \caption[Experiment 1]{\label{fig:exp1}
    \textbf{Gradient descent in action space (Experiment 1, $n = 20$).}
    (\textbf{a}) Each human subject $H$ is instructed to provide manual input $h$ to make a black bar on a computer display as small as possible. The bar's height represents the value of a prescribed cost $c_H$.
    (\textbf{b}) The machine $M$ has its own cost $c_M$ chosen to yield game-theoretic equilibria that are distinct from each other and from each player's global optima. The machine knows its cost and observes human actions $h$.
    In this experiment, the machine updates its action by gradient descent on its cost $\frac{1}{2}m^2-hm+h^2$ with adaptation rate $\alpha$.
    (\textbf{c}) Median joint actions for each machine adaptation rate $\alpha$ overlaid on game-theoretic equilibria and best-response (BR) curves that define the Nash and Stackelberg equilibria (NE and SE, respectively).
    (\textbf{d}) Action distributions for each machine adaptation rate displayed by box-and-whiskers plots showing 5th, 25th, 50th, 75th, and 95th percentiles.
    Statistical significance ($*$) 
    determined by 
    comparing 
    to NE (shown below distributions) and SE (shown above distributions) 
    using two-sided $t$-tests ($^*P \leq 0.05$).
    (\textbf{e}) Cost distributions for each machine adaptation rate displayed using box plots with error bars showing 25th, 50th, and 75th percentiles. 
    (\textbf{f,g}) One- and two-dimensional histograms of actions for different adaptation rates ($\alpha \in \set{\text{0,0.003}}$ in (f), $\alpha\in\set{\text{0.3, 1}}$ in (g)) with game-theoretic equilibria overlaid (NE in (f), SE in (g)).
}


==> fig/tex_exp2v5.tex <==
\centering
\includegraphics[width=\textwidth]{fig/fig_exp2v5.pdf}
  \caption[Experiment 2]{\label{fig:exp2}
  \textbf{Conjectural variation in policy space (Experiment 2, $n = 20$).}
  Experimental setup and costs are the same as~\figref{exp1}{a,b}
  except that the machine uses a different adaptation algorithm:
  in this experiment
  $M$ iteratively implements and updates affine policies $m = L_M h$, $m = L_M + \delta$ to measure and best-respond to conjectures of the human's policy.
  (\textbf{a}) Median actions, conjectures, and policies for each conjectural variation iteration $k$ overlaid on game-theoretic equilibria corresponding to best-responses (BR) at initial and limiting iterations (BR$_0$ and BR$_\infty$, respectively) predicted from Stackelberg and Consistent Conjectural Variations equilibria of the game (SE and CCVE), respectively. 
  (\textbf{b}) Action distributions for each iteration displayed by box-and-whiskers plots as in~\figref{exp1}d, 
  with statistical significance ($*$) 
  analogously determined using the same tests by 
  comparing 
  to SE (shown below distributions) and CCVE (above).
  (\textbf{c}) Policy slope distributions for each iteration displayed with the same conventions as (b); 
  note that the sign of the top $y$-axis is reversed for consistency with other plots.
  Statistical significance ($*$) 
  determined as in (b) by 
  comparing 
  to initial (shown below distributions) and limiting (above) best-responses 
  using two-sided $t$-tests ($^*P \leq 0.05$).
  (\textbf{d}) Cost distributions 
  for each iteration displayed using box-and-whiskers plots as in~\figref{exp1}e.
  (\textbf{e,f}) One- and two-dimensional histograms of actions for different iterations ($k=0$ in (e), $k=9$ in (f)) with policies and game-theoretic equilibria overlaid (SE and BR$_0$ in (e), CCVE and BR$_\infty$ in (f)).
  (\textbf{g})
  Error between measured %($\widetilde{L}_H$) 
  and theoretically-predicted %($L_H$) 
  machine conjectures about human policies at each iteration displayed as box-and-whiskers plots as in (b,c).
}


==> fig/tex_exp3_init.tex <==
\centering
\includegraphics[width=\textwidth]{fig/fig_exp3_init.pdf}
  \caption[Experiment 3 with different initial policy]{\label{fig:exp3-other-init}
  \footnotesize
  \textbf{Experiment 3 with different initial policy} ($n=20$): gradient descent in policy space for a different initial machine policy.
  (\textbf{A}) Game-theoretic equilibria and best-response functions.
  (\textbf{B}) Decision vector distributions.
  (\textbf{C}) Cost distributions.
  (\textbf{D}) Machine policy slopes.
  (\textbf{E}) Estimation error of machine policy gradients.
  Action IQR in (B) contains the machine's minimum at each iteration 4 to 9.
  Machine's policy slope distribution IQR in (D) reaches the theoretically-predicted slope that would yield the machine's minimum as the game outcome.
  The machine's policy gradient IQR in (E) contains the theoretical gradient at every policy gradient iteration.
  }


==> fig/tex_exp3_other.tex <==
\centering
\includegraphics[width=\textwidth]{fig/fig_exp3_other.pdf}
  \caption[Experiment 3 with different machine optima]{\label{fig:exp3-other-optima}
  \footnotesize
  \textbf{Experiment 3 with different machine optima} ($n=18$): gradient descent in policy space for differing machine optima.
  (\textbf{A}) Game-theoretic equilibria and best-response functions.
  (\textbf{B}) Decision vector distributions.
  (\textbf{C}) Cost distributions.
  (\textbf{D}) Machine policy slopes.
  (\textbf{E}) Estimation error of machine policy gradients.
 % Action IQR in (B) contains the machine's minimum at each iteration 4 to 9.
 % Machine's policy slope distribution IQR in (D) reaches the theoretically-predicted slope that would yield the machine's minimum as the game outcome.
%  The machine's policy gradient IQR in (F) contains the theoretical gradient at every policy gradient iteration.
%  (\textbf{A}) Game-theoretic equilibria and best-response functions.
%  (\textbf{B}) Decision vector distributions; violin plots with quartiles.
%  (\textbf{C}) Cost distributions; box plots with quartiles.
%  (\textbf{D}) Machine policy slopes; violin plots with quartiles.
%  (\textbf{E}) Estimation error of machine policy gradients; box plots with quartiles.
%  (Conventions for violin and box plots as in~\figref{exp1}.)
%  Action IQR in (B) contains the Stackelberg equilibrium only in the first two policy gradient iterations, but contains the machine's minimum at each iteration 6 to 9.
%  Machine's policy slope distribution IQR in (D) contains the Stackelberg slope only in the first two policy gradient iterations, and never reaches the theoretically-predicted slope that would yield the machine's minimum as the game outcome,
%  although the machine's policy gradient IQR in (F) contains the theoretical gradient at every policy gradient iteration.
  Action IQR in (B) contains the machine's minimum at each iteration 7 to 9.
  Machine's policy slope distribution IQR in (D) approaches the theoretically-predicted slope that would yield the machine's minimum as the game outcome.
      }


==> fig/tex_exp3v5.tex <==
\centering
\includegraphics[width=\textwidth]{fig/fig_exp3v5.pdf}
  \caption[Experiment 3]{\label{fig:exp3}
  \textbf{Gradient descent in policy space (Experiment 3, $n = 20$).} 
  Experimental setup and costs are the same as~\figref{exp1}a,b except that the machine uses a different adaptation algorithm:
  in this experiment, $M$ iteratively implements linear policies $m = L_M h$, $m = (L_M + \Delta)h$ to measure the gradient of its cost with respect to its policy slope parameter $L_M$ and updates this parameter to descend its cost landscape.
  (\textbf{a}) 
  Median actions and policies for each policy gradient iteration $k$ overlaid on game-theoretic equilibria corresponding to machine best-responses (BR) at initial and limiting iterations (BR$_0$ and BR$_\infty$, respectively) predicted from the Stackelberg equilibrium (SE) and the machine's global optimum (RSE), respectively.
  (\textbf{b}) 
  Action distributions for each iteration displayed by box-and-whiskers plots as in~\figref{exp1}d, with statistical significance ($*$) analogously determined using the same tests by comparing to SE (shown above distributions) and $M$'s optimum (shown below distributions)
  using two-sided $t$-tests ($^*P \leq 0.05$);
  (\textbf{c}) 
  Policy slope distributions for each iteration displayed with the same conventions as (b); 
  note that the sign of the top subplot's $y$-axis is reversed for consistency with other plots.
  Statistical significance ($*$) determined as in (b) by comparing to SE (shown above distributions) 
  and RSE (below)
  using two-sided $t$-tests ($^*P \leq 0.05$).
  (\textbf{d}) 
  Cost distributions for each iteration displayed using box-and-whiskers plots as in~Figures~\ref{fig:exp1}e and~\ref{fig:exp2}d. 
  (\textbf{e,f}) One- and two-dimensional histograms of actions for different iterations ($k=0$ in (e), $k=9$ in (f)) with policies and game-theoretic equilibria overlaid (SE in (e), RSE in (f)).
  (\textbf{g}) 
  Error between measured and theoretically-predicted policy slopes at each iteration displayed as box-and-whiskers plots as in (b,c).
}


==> fig/tex_overviewv5.tex <==
\centering
\includegraphics[width=\textwidth]{fig/fig_overviewv5.pdf}
  \caption[Co-adaptation game between human and machine]{\label{fig:overview}
  \scriptsize
  \textbf{Overview of co-adaptation experiment between human and machine.} 
 Human subject $H$ is instructed to provide manual input $\actH$ to make a black bar on a computer display as small as possible.
The machine $M$ has its own prescribed cost $\costM$ chosen to yield game-theoretic equilibria that are distinct from each other and from each player's global optima.
  (\textbf{a}) Joint action space illustrating game-theoretic equilibria and response functions determined from the costs prescribed to human and machine: \emph{global {\optima}} defined by minimizing with respect to both variables; \emph{best-response} functions defined by fixing one variable and minimizing with respect to the other. 
   Machine plays different strategies in three experiments:
   (\textbf{b}) gradient descent in \emph{Experiment 1};
   (\textbf{c})  conjectural variation in \emph{Experiment 2};
   (\textbf{d})  policy gradient descent in \emph{Experiment 3}.
  }


==> fig/tex_pareto.tex <==
\centering
\includegraphics[width=\textwidth]{fig/fig_pareto.pdf}
  \caption[Comparing Pareto optimality with conjecture consistency]{\label{fig:pareto-consistency}   \scriptsize
  \textbf{Comparing Pareto optimality with conjecture consistency}
    \textbf{(\sf A)} 
    The analytical solution for the continuum of equilibria where the human has a consistent conjecture about the machine and vice versa, compared with the Pareto optimal points.
  \textbf{(\sf B)} The median actions from Experiments 2 and 3 coincide with the ellipse that corresponds to the human having a consistent conjecture about the machine. 
  }
  
  


==> fig/tex_sim.tex <==
\centering
\includegraphics[width=\textwidth]{fig/fig_sim.pdf}
  \caption[Simulations of Experiments 1, 2 and 3]{\label{fig:sim-quad}
  \footnotesize
  \textbf{Simulations of Experiments 1, 2 and 3}: Solid lines and dots are the simulation data, overlaid on violin plots from main paper. Dashed lines are analytical predictions.
  (\textbf{A}) Gradient descent in action space.
  (\textbf{B}) Conjectural variation in policy space.
  (\textbf{C}) Gradient descent in policy space.
  }

